FvOR: Robust Joint Shape and Pose Optimization for Few-view Object Reconstruction

Reconstructing an accurate 3D object model from a few image observations remains a challenging problem in computer vision. State-of-the-art approaches typically assume accurate camera poses as input, which could be difficult to obtain in realistic settings. In this paper, we present FvOR, a learning-based object reconstruction method that predicts accurate 3D models given a few images with noisy input poses. The core of our approach is a fast and robust multi-view reconstruction algorithm to jointly refine 3D geometry and camera pose estimation using learnable neural network modules. We provide a thorough benchmark of state-of-the-art approaches for this problem on ShapeNet. Our approach achieves best-in-class results. It is also two orders of magnitude faster than the recent optimization-based approach IDR. Our code is released at \url{https://github.com/zhenpeiyang/FvOR/}

==> Tables/shapenet_init_shape.tex <==

\begin{table*}
\centering
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{r|cccc|cc}
\toprule
\multirow{2}{*}{} & \multicolumn{4}{c|}{w/o GT  Pose}&  \multicolumn{2}{c}{w/ GT  Pose} \\

&OccNet~\cite{mescheder2019occupancy} & OccNet$^\dagger$~\cite{apple,mescheder2019occupancy}&Pix2Vox++~\cite{xie2020pix2vox++} & \ouralg(Ours) & 3D43D~\cite{apple} & \ouralg  w. GT Pose \\ \hline
Mean  & 0.593 / 1.9 / 0.840  & 0.621 / 2.7 / 0.854 & 0.455/-/-& \textbf{0.735} / \textbf{0.8} / \textbf{0.914} &0.749 / 0.7 / 0.906&\textbf{0.78} / \textbf{0.6} / \textbf{0.928}\\ 

\bottomrule
\end{tabular}
}
\vspace{-0.1in}
\caption{Quantitative results of few-view 3D reconstruction on the ShapeNet dataset. The numbers in each cell is (IoU$\uparrow$ / Chamfer-L1$\downarrow$ / Normal consistency$\uparrow$). OccNet~\cite{mescheder2019occupancy} uses a single view. Other methods use 5 views. The last two columns show methods that use GT camera poses. Results for OccNet/OccNet$^\dagger$/3D43D are copied  from the original papers. Chamfer-L1 is multipled by 100~\cite{mescheder2019occupancy}. We leave the per-category results to the supp.. }
\label{table:shapenet-shape-init}
\vspace{-0.1in}
\end{table*}

==> symbols.tex <==
\let \bs = \boldsymbol
%\newcommand{\classset}{\mathcal{C}}
\let \set = \mathcal

\newcommand{\pos}{\mathbf{p}}
\newcommand{\vertex}{\bs{v}}
\newcommand{\edge}{\bs{e}}
\newcommand{\pred}{0}
\newcommand{\init}{\textup{init}}
\newcommand{\pose}{\textup{pose}}
\newcommand{\GMM}{M}
\newcommand{\GAMMA}{\Gamma}
\newcommand{\graph}{\mathcal{G}}
\newcommand{\vertexset}{\mathcal{V}}
\newcommand{\edgeset}{\mathcal{E}}
\newcommand{\edgeweightset}{\mathcal{W}}
\newcommand{\edgeweight}{w}
\newcommand{\normalizededgeweight}{\hat{w}}

\newcommand{\gt}{\textup{gt}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\klloss}{\loss_{KL}}

\newcommand{\argmin}{\arg\min}

\newcommand{\ps}{\mathcal{P}}

\DeclareMathOperator{\Tr}{Tr}

\newcommand{\smooth}{\textup{smooth}}
\newcommand{\p}{\bs{p}}
\newcommand{\q}{\bs{q}}
\newcommand{\ro}{\bs{r}} 
\newcommand{\tn}{\bs{t}} % translation
\newcommand{\n}{\bs{n}} % normal
\newcommand{\om}{\bs{\omega}} % Lie algebra

\newcommand{\vf}{\bs{v}} % vertex feature
\newcommand{\ef}{\bs{e}} % edge feature

\newcommand{\T}{\bs{T}} % Transformation

\newcommand{\R}{\mathcal{R}}
\newcommand{\Q}{\bs{Q}}
\newcommand{\W}{\bs{W}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\skewm}[1]{\left[#1\right]_{\times}}

\newcommand{\primitive}{p}

